UniVA: Universal Video Agent towards Open-Source Next-Generation Video Generalist

While specialized AI models excel at isolated video tasks like generation or understanding, real-world applications demand complex, iterative workflows that combine these capabilities. To bridge this gap, we introduce UniVA, an open-source, omni-capable multi-agent framework for next-generation video generalists that unifies video understanding, segmentation, editing, and generation into cohesive workflows. UniVA employs a Plan-and-Act dual-agent architecture that drives a highly automated and proactive workflow: a planner agent interprets user intentions and decomposes them into structured video-processing steps, while executor agents execute these through modular, MCP-based tool servers (for analysis, generation, editing, tracking, etc.). Through a hierarchical multi-level memory (global knowledge, task context, and user-specific preferences), UniVA sustains long-horizon reasoning, contextual continuity, and inter-agent communication, enabling interactive and self-reflective video creation with full traceability. This design enables iterative and any-conditioned video workflows (e.g., text/image/video-conditioned generation $\rightarrow$ multi-round editing $\rightarrow$ object segmentation $\rightarrow$ compositional synthesis) that were previously cumbersome to achieve with single-purpose models or monolithic video-language models. We also introduce UniVA-Bench, a benchmark suite of multi-step video tasks spanning understanding, editing, segmentation, and generation, to rigorously evaluate such agentic video systems. Both UniVA and UniVA-Bench are fully open-sourced, aiming to catalyze research on interactive, agentic, and general-purpose video intelligence for the next generation of multimodal AI systems. (https://univa.online/)

==> promtable.tex <==





\RequirePackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} 
\def\ie{\emph{i.e}\onedot} 
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


\definecolor{adptorange}{RGB}{248, 205, 172}
\definecolor{cmpblue}{RGB}{189, 215, 238}
\definecolor{cmpblue}{RGB}{189, 215, 238}

\definecolor{our_red}{RGB}{232,157,160}
\definecolor{our_blue}{RGB}{136,206,230}
\definecolor{our_orange}{RGB}{246,200,168}
\definecolor{our_green}{RGB}{178,211,164}

\definecolor{attn_code0}{RGB}{247,215,200}
\definecolor{attn_code1}{RGB}{238,169,139}
\definecolor{mlp_code0}{RGB}{204,201,221}
\definecolor{mlp_code1}{RGB}{102,95,153}

\definecolor{token_blue}{RGB}{84, 120, 140}
\def\blue#1{\textbf{\color{our_blue} #1}} %in Table
\def\red#1{\textbf{\color{our_red} #1}} %in Table
\def\green#1{\textbf{\color{our_green} #1}} %in Table
\def\orange#1{\textbf{\color{our_orange} #1}} %in Table
\def\tokenblue#1{\textbf{\color{token_blue} #1}} %in Table

% \newcommand{\xmark}{\ding{55}}
% \newcommand{\cmark}{\ding{51}}

\def\vx{{\bm{x}}}

\newlength\savewidth\newcommand\shline{\noalign{\global\savewidth\arrayrulewidth \global\arrayrulewidth 1pt}\hline\noalign{\global\arrayrulewidth\savewidth}}
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}

\newcolumntype{x}[1]{>{\centering\arraybackslash}p{#1pt}}
\newcolumntype{y}[1]{>{\raggedright\arraybackslash}p{#1pt}}
\newcolumntype{z}[1]{>{\raggedleft\arraybackslash}p{#1pt}}

\renewcommand{\paragraph}[1]{\vspace{1mm}\noindent\textbf{#1}}

\newcommand\hshline{\noalign{\global\savewidth\arrayrulewidth
  \global\arrayrulewidth 0.5pt}\hline\noalign{\global\arrayrulewidth\savewidth}}

\setlength{\abovecaptionskip}{1pt}

\renewcommand{\paragraph}[1]{\vspace{1.25mm}\noindent\textbf{#1}}

\definecolor{codeblue}{rgb}{0.25, 0.5, 0.5}
\definecolor{codekw}{rgb}{0.35, 0.35, 0.75}
\lstdefinestyle{Pytorch}{
    language = Python,
    backgroundcolor = \color{white},
    basicstyle = \fontsize{9pt}{8pt}\selectfont\ttfamily\bfseries,
    columns = fullflexible,
    aboveskip=1pt,
    belowskip=1pt,
    breaklines = true,
    captionpos = b,
    commentstyle = \color{codeblue},
    keywordstyle = \color{codekw},
}

\definecolor{green}{HTML}{009000}
\definecolor{red}{HTML}{ea4335}
\newcommand{\better}[1]{\textcolor{green}{$\uparrow\,$#1}}
\newcommand{\worse}[1]{\textcolor{red}{$\downarrow\,$#1}}
\newcommand{\betterinv}[1]{\textcolor{green}{$\downarrow\,$#1}}
\newcommand{\worseinv}[1]{\textcolor{red}{$\uparrow\,$#1}}

\newcommand{\eqcontrib}{\clubsuit}
\newcommand{\correspond}{\spadesuit}

\newcommand{\ours}{\textsc{VL-Cogito}\xspace}

\newtcolorbox{promptblock}{
    colback=gray!5,
    colframe=gray!15,
    boxrule=0.5pt,
    arc=3pt,
    left=12pt,
    right=12pt,
    top=8pt,
    bottom=8pt,
    boxsep=8pt,
    breakable
}


% ====================================

\definecolor{hidden-draw}{RGB}{20,68,106}
\definecolor{hidden-pink}{RGB}{255,245,247}

\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
  frame=single,
  breaklines=true,
  keepspaces=true
  % xleftmargin=.2\textwidth，xrightmargin=.2\textwidth
}

\urlstyle{same}
\usepackage{makecell}
% \usepackage[dvipsnames]{xcolor}
\newtheorem{definition}{Definition}

\newtheorem{defn}{\hspace{-1mm} Definition}
\newtheorem{remark}{\noindent \textbf{Remark}}
\newtheorem{discussion}{\noindent \textbf{Discussion}}



\usepackage[edges]{forest}
\definecolor{hiddendraw}{RGB}{205, 44, 36}
\definecolor{hidden-blue}{RGB}{194,232,247}
\definecolor{hidden-orange}{RGB}{243,202,120}
\definecolor{hidden-yellow}{RGB}{242,244,193}
\definecolor{uclablue}{rgb}{0.15, 0.45, 0.68}
\definecolor{lightgrey}{RGB}{201,203,209}


\usepackage{hyperref}
\hypersetup{
    breaklinks,
    colorlinks=true,
    % linkcolor=uclablue,
    citecolor=uclablue,
    % filecolor=uclablue,      
    urlcolor=uclablue,
}

\tikzstyle{mybox}=[
    rectangle,
    draw=hiddendraw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    ]


\newcommand{\cmark}{{\textcolor{c1}\Checkmark}}
\newcommand{\xmark}{{\textcolor{c2}\XSolidBrush}}







% Section - Larger bold font
\renewcommand*\l@section[2]{%
  \@dottedtocline{1}{0em}{2.3em}{\bfseries #1}{#2}
}
% Subsection - Normal bold font
\renewcommand*\l@subsection[2]{%
  % \@dottedtocline{2}{1.5em}{2.8em}{\bfseries\small #1}{#2}
  \@dottedtocline{2}{1.5em}{2.8em}{\small #1}{#2}
}
% Subsubsection - Normal font
\renewcommand*\l@subsubsection[2]{%
  \@dottedtocline{3}{3.0em}{3.2em}{\small #1}{#2}
}

